Detecting and Identifying Selection Structure in Sequential Data

We argue that the selective inclusion of data points based on latent objectives is common in practical situations, such as music sequences. Since this selection process often distorts statistical analysis, previous work primarily views it as a bias to be corrected and proposes various methods to mitigate its effect. However, while controlling this bias is crucial, selection also offers an opportunity to provide a deeper insight into the hidden generation process, as it is a fundamental mechanism underlying what we observe. In particular, overlooking selection in sequential data can lead to an incomplete or overcomplicated inductive bias in modeling, such as assuming a universal autoregressive structure for all dependencies. Therefore, rather than merely viewing it as a bias, we explore the causal structure of selection in sequential data to delve deeper into the complete causal process. Specifically, we show that selection structure is identifiable without any parametric assumptions or interventional experiments. Moreover, even in cases where selection variables coexist with latent confounders, we still establish the nonparametric identifiability under appropriate structural conditions. Meanwhile, we also propose a provably correct algorithm to detect and identify selection structures as well as other types of dependencies. The framework has been validated empirically on both synthetic data and real-world music.

==> sections/appx_alg.tex <==
\section{Full Algorithm}

\begin{algorithmic}[1]
	% \caption{Learning selection structure (Part 1)}
	\label{alg:global}
	\STATE \textbf{Input:} Data $\mathbf{X}$;
	\STATE \textbf{Output:} A complete causal graph $\mathcal{G}$;
    \STATE Set $N$ as the number of variables in $\X$;
    \STATE Initialize two empty lists as $\mathcal{L} \coloneqq [\cdot]$ and $\mathcal{R} \coloneqq [\cdot]$;
    \STATE Initialize an edge set with time-oriented structures $\mathcal{E} \coloneqq \{1 \rightarrow 2, 2 \rightarrow 3, \dots, N-1 \rightarrow N\}$;
    \STATE Initialize a set of vertices $\mathcal{V} \coloneqq \{1,2,\cdots,N\}$;

    % detect spurious pairs
    \FOR{$l$ in $\{N-1, N-2, \cdots, 1\}$}
        \STATE Set $i \coloneqq 1$, $j \coloneqq i+l$;
        \WHILE{$j \leq N$}
            \IF{$X_i \notindependent X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$}
                \IF{$\forall k \in \mathcal{R}[i], X_i \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}, X_{j+1}, X_k\}$}
                    \STATE $\mathcal{L}$.append$(i)$;
                    \STATE $\mathcal{R}[i]$.append$(j)$;
                \ENDIF
            \ENDIF
            \STATE Set $i \coloneqq i+1$, $j \coloneqq i+l$;
        \ENDWHILE
    \ENDFOR


    % detect selection and higher-order causal inference
    \STATE Set $u \coloneqq 0$;
    \FOR{$i \in ReverseSorted(\mathcal{L})$}
        \FOR{$j \in ReverseSorted(\mathcal{R}[i])$}
            \STATE Set $k = j-1$;
            \WHILE{$k \in \mathcal{R}[i]$ and $k > i+1$}
                \STATE $k \coloneqq k-1$
            \ENDWHILE
            \STATE $\mathbf{T} = \{X_v$, where $(X_p,X_v)_s \in \mathcal{E}$\} 
            % \STATE $\mathbf{T}_2 = \{v \in R[i] \cup R[j]$, where $(X_i,X_v)_s$ or $(X_j,X_v)_s$\} 

            % \IF {$X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j\}$ and $\forall v \in \mathbf{T}, X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}$}
            \IF {$X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, \mathbf{T}\}$}
                % \IF {$X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}\}$ and $\forall v \in \mathbf{T}, X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_v\}$}
                \IF {$X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_{j+1}, \mathbf{T}\}$}
                    \STATE Add to $\mathcal{E}$ an edge $i \rightarrow j$;
                    \STATE Add to $\mathcal{E}$ edges $i \rightarrow s_u$ and $j \rightarrow s_u$;
                    \STATE Set $u \coloneqq u+1$;
                    \IF {$j-1 \in \mathcal{R}[i]$}
                        \STATE $\mathcal{R}[i]$.remove$(j-1)$;
                    \ENDIF
                % \ELSIF{$j \notin \mathcal{R}[i] \cap \mathcal{R}[i-1]$}
                \ELSE
                    \STATE Add to $\mathcal{E}$ an edge $i \rightarrow j$;
                \ENDIF
            \ELSE
                \STATE Add to $\mathcal{E}$ edges $i \rightarrow s_u$ and $j \rightarrow s_u$;
                \STATE Set $u \coloneqq u+1$;
                % \IF{$j+1 \in \mathcal{R}[i]$}
                %     \STATE $\mathcal{R}[i]$.remove$(j)$ % remove fake j before both (i,j)_{sx/c}
                % \ELSE         
                %     \STATE Add to $\mathcal{E}$ edges $i \rightarrow s_u$ and $j \rightarrow s_u$;
                %     \STATE Set $u \coloneqq u+1$;
                % \ENDIF
            \ENDIF
        \ENDFOR
    \ENDFOR
    
    % detect confounded pairs
    \STATE Set $u \coloneqq 0$;
    \FOR{$j$ in $\{N, N-1 \cdots, 3\}$}
        \FOR{$i$ in $\{N-1, N-2 \cdots, 2\}$}
            \STATE $\mathbf{T} = \{X_v$, where $(X_{i-1},X_v)_s$, $(X_{i},X_v)_s$, or $(X_{i+1},X_v)_s$, $v>j$\}
            \IF{$i \rightarrow j$ and $i-1 \rightarrow j$}
                \IF{$X_{i-1} \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus \{i-1,i\}}, X_{j+1},\mathbf{T}\}$}
                    \STATE Add to $\mathcal{E}$ edges $i-1 \rightarrow j$ and $i \rightarrow j$;
                    % \IF{$X_{i-1} \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus \{i-1,i\}},\mathbf{T}\}$}
                    % % \IF{$\forall k \in \mathcal{R}[i-1]\cup\mathcal{R}[i]$ and $k > j$, $X_{i-1} \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus \{i-1,i\}}, \mathbf{X}_{\mathcal{R}[i+1]}, X_k\}$}
                    %     \STATE Add to $\mathcal{E}$ edges $i-1 \rightarrow j$ and $i \rightarrow j$;
                    %     % \STATE $\mathcal{R}[i-1]$.remove$(j)$;
                    % \ELSE
                    %     \STATE Add to $\mathcal{E}$ edges $c_u \rightarrow i$ and $c_u \rightarrow j$;
                    %     \STATE Remove $i-1 \rightarrow j$ and $i \rightarrow j$ from $\mathcal{E}$
                    %     \STATE Set $u \coloneqq u+1$; 
                    % \ENDIF
                    
                \ELSE
                    \STATE Add to $\mathcal{E}$ edges $c_u \rightarrow i$ and $c_u \rightarrow j$;
                    \STATE Remove $i-1 \rightarrow j$ and $i \rightarrow j$ from $\mathcal{E}$
                    \STATE Set $u \coloneqq u+1$;
                \ENDIF
            \ENDIF
        \ENDFOR
    \ENDFOR


	\STATE {\bfseries Return} $\mathcal{G} = \{\mathcal{V}, \mathcal{E}\}$;
\end{algorithmic}

==> sections/appx_old.tex <==
\section{Proofs}

\subsection{Proof of Theorem \ref{thm:1}}
\label{sec:proof_thm_1}

\thmI*

\begin{proof}
% Since we assume that there are no latent confounders in the ground-truth causal graph $\mathcal{G}$, our goal is to identify all selection pairs $(X_i, X_j)_s$ ($X_i \rightarrow S_k \leftarrow X_j$) and direct relations ($X_i \rightarrow X_j$). Based on Alg. XX, we first identify all dependent pairs $(X_i, X_j)_d$ and then determine their types.

% According to [Alg. xxx], given any pair of variables $X_i$ and $X_j$, we first detect whether $X_i$ is conditionally dependent of $X_j$ given $\mathbf{X}_{\text{Pre}(j) \setminus i}$, where $\text{Pre}(j)$ denotes indices smaller than $j$ ($\{1,2,\cdots,j-1\}$). If $X_i \notindependent X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$, there are two possible cases:

% \begin{itemize}
%     \item There exists a dependent pair $(X_i, X_j)_d$. Because of faithfulness, the dependent pair implies $X_i \notindependent X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$. Note that since $\mathbf{X}$ is under selection bias, the selection variables are always being conditioned, i.e., $X_i$ is always d-connected with $X_j$ for a selection pair $(X_i, X_j)_d$ ($X_i \rightarrow S_k \leftarrow X_j$, $S_k \in \mathbf{S}$).
    
%     \item There does not exist a dependent pair $(X_i, X_j)_d$, but a selection pair $(X_i, X_v)_s$ where $v > j$. Since there are no latent confounders, conditioning on $\mathbf{X}_{\text{Pre}(j) \setminus i}$ blocks all paths starting from any variables in the set $\mathbf{X}_{\text{Pre}(j) \setminus i}$. Thus, the only type of paths between $X_i$ and $X_j$ that are not $(X_i, X_j)_d$ is $X_i \cdots X_v \cdots \X_{j}$, where $v > j$.
    
%     In addition, given assumption \ref{assum:t1a1}, it is impossible for any path
% \end{itemize}


\end{proof}


\subsection{Proof of Theorem \ref{thm:2}}
\label{sec:proof_thm_2}

\thmII*

\begin{proof}
    We prove the identifiability of the causal graph by showing that the algorithm \ref{alg:global} identifies all selection pairs, direct relations, and confounded pairs. Consistent with the three stages of the algorithm, the proof is divided into the following three stages:
    \begin{itemize}
        \item \textbf{Stage I}: Identifying dependent pairs (selection pairs, direct relations, and confounded pairs) together with several spurious structures.
        \item \textbf{Stage II}: Identifying selection pairs, dependent pairs that are both selection pairs and direct relations, and direct relations, while while removing some spurious structures.
        \item \textbf{Stage III}: Identifying confounded pairs while removing all spurious structures.
    \end{itemize}

    \textbf{Stage I.} \ \
    We first show that, after Lines 1-18, the identified sets of variable pairs, denoted as $\mathbf{E}_1$, only consists of the following types of cases:
    \begin{itemize}
        \item All selection pairs $(X_i, X_j)_s$ in the ground-truth causal graph. 
        % Since $\mathbf{X}$ is under selection bias, the selection variables are always being conditioned. Thus, there is always a d-connected path between $(X_i, X_j)_s$, i.e., $\{X_i \rightarrow S \leftarrow X_j\}$, for any $X_i, X_j \in \mathbf{X}$. We denote $S$ as the corresponding selection variable in $\mathbf{S}$.
        \item All direct relations $(X_i, X_j)_x$ in the ground-truth causal graph.
        \item All confounded pairs $(X_i, X_j)_c$ in the ground-truth causal graph.
        \item All pairs of variables $(X_i, X_j)$ that there exist confounded pairs $(X_{i+1}, X_j)_c$ in the ground-truth causal graph.
        % \item All dependent pairs that are both selection pairs and direct relations, i.e., $(X_i, X_j)_{\{s,x\}}$, in the ground-truth causal graph.
        \item All pairs of variables $(X_i, X_j)$ that there exists $(X_i, X_{j+1})$ that is both a selection pair and a direct relation in the ground-truth causal graph.
        % \item All pairs of variables $(X_i, X_j)$ that there exist $(X_i, X_{j+1})_{\{s\}}$ and $(X_{i+1}, X_{j+1})_c$ in the ground-truth causal graph.
    \end{itemize}
    For a variable pair $(X_i, X_j)$, we discuss all potential cases for the paths between $X_i$ and $X_j$ as follows. We denote $X_k$ as the observed variable closest to $X_i$.  
    
    % because of faithfulness, the conditional independence $X_i \notindependent X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$ implies that $X_i$ and $X_j$ are d-connected by $\mathbf{X}_{\text{Pre}(j) \setminus i}$.
    \begin{itemize}
        \item $(X_i, X_j)$ is a dependent pair. In this case, $X_i$ is d-connected with $X_j$ given any conditioning set, thus  $X_i \notindependent X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$ and $(X_i, X_j)_d \in \mathbf{E}_1$.
        
        \item $\{X_i \cdots \leftarrow X_k \cdots X_j\}$, where $k<i$. Since $X_k \in \mathbf{X}_{\text{Pre}(j) \setminus i}$, this path is d-connected if and only if $X_k$ is a collider on the path. However, $X_k$ cannot be a collider because of $\{X_i \leftarrow X_k\}$. Thus, $X_i \indep X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$ and $(X_i, X_j)_d \notin \mathbf{E}_1$.
        
        \item $\{X_i \cdots \rightarrow X_k \cdots X_j\}$, where $k<i$. Because of assumption \ref{assum:t2a1}, $\{X_i \rightarrow X_k\}$ is impossible. Thus, there must be a confounded pair $\{X_i, X_k\}_c$. Because of assumption \ref{assum:t2a2}, $X_k$ cannot be caused by another confounder or observed variable via higher-order direct relation. Therefore, $X_k$ is not a collider, and we have $X_i \indep X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$ ($X_k \in \mathbf{X}_{\text{Pre}(j) \setminus i}$ and thus $(X_i, X_j)_d \notin \mathbf{E}_1$.
        
        \item $\{X_i \cdots \leftrightarrow X_k \cdots X_j\}$, where $k<i$ and $\leftrightarrow$ means both tails and arrow heads exist. Because of assumption \ref{assum:t2a1}, $\{X_i \rightarrow X_k\}$ is impossible. Thus, there must be a confounded pair $\{X_k, X_i\}_c$. Because of assumption \ref{assum:t2a2}, $(X_k, X_i)$ cannot be a selection pair or direct relation, and $X_k$ cannot be caused by another confounder or observed variable via higher-order direct relation. We further discuss the following cases:
        \begin{itemize}
            \item $X_k$ is a collider. For $X_k$ to be a collider, the only case is $\{X_{k-1} \rightarrow X_k \leftarrow C \rightarrow X_i\}$, where $C$ as the corresponding latent confounder in $\mathbf{C}$. In that case, $X_{k-1} \in \mathbf{X}_{\text{Pre}(j) \setminus i}$ cannot be a collider on the path. Thus, we have $X_i \indep X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$.
            \item $X_k$ is not a collider. Then we have $X_i \indep X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$ ($X_k \in \mathbf{X}_{\text{Pre}(j) \setminus i}$) and thus $(X_i, X_j)_d \notin \mathbf{E}_1$.
        \end{itemize}
        
        \item $\{X_i \cdots \leftarrow X_k \cdots X_j\}$, where $k>i$. Based on this, we discuss the following cases: 
        \begin{itemize}
            \item The case where $i < k < j$. Because of assumption \ref{assum:t2a1}, $\{X_i \leftarrow X_k\}$ is impossible. Thus, there must be a selection pair $\{X_i, X_k\}_s$, and $X_k$ must not be a collider. Since $\mathbf{X}_{\text{Pre}(j) \setminus i}$ is the condition set and $X_k \in \mathbf{X}_{\text{Pre}(j) \setminus i}$, we have $X_i \indep X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$ ($X_k \in \mathbf{X}_{\text{Pre}(j) \setminus i})$ and thus $(X_i, X_j)_d \notin \mathbf{E}_1$.
            \item The case where $k > j$. Because of assumption \ref{assum:t2a1}, $\{X_i \leftarrow X_k\}$ is impossible. Thus, there must be a selection pair $\{X_i, X_k\}_s$, and $X_k$ must not be a collider. Since $k > j$, $X_k$ is not in the conditioning set $\mathbf{X}_{\text{Pre}(j) \setminus i}$. However, the index $k$ for any selection pair $\{X_i, X_k\}_s$, where $k>j$, has already been included in $\mathcal{R}[i]$ according to the order of tests in the algorithm (Lines 7-9, 16). Therefore, there is the conditional independence $X_i \indep X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}, X_{j+1}, X_k\}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$.
        \end{itemize}

        \item $\{X_i \cdots \rightarrow X_k \cdots X_j\}$, where $k>i$. Based on this, we discuss the following cases:
        \begin{itemize}
            \item The case where $i < k < j$. Since $\mathbf{X}_{\text{Pre}(j) \setminus i}$ is the condition set and $X_k \in \mathbf{X}_{\text{Pre}(j) \setminus i}$, $X_k$ must be a collider for the path to be d-connected. On the path, let us denote the $X_p$ as the observed variable closest to $X_k$ other than $X_i$. Thus, we must have $\{X_k \leftarrow \cdots X_p\}$ on the path. We further have the following cases:
                \begin{itemize}
                    \item The case where $p < k$. If $p < k$, we have $p < i$ as $p \neq i$. Since $\{X_k \leftarrow \cdots X_p\}$, $(X_k, X_p)$ is either a confounded pair or direct relation. We further discuss the following cases:
                    \begin{itemize}
                        \item If $(X_k, X_p)$ is a confounded pair, because $X_p$ cannot be caused by another confounder (assumption \ref{assum:t2a2}), the only case for $X_p$ to also be a collider is $\{X_k \leftarrow C \rightarrow X_p \leftarrow X_{p-1}$. Thus, $X_{p-1}$ must not be a collider, and $X_i \indep X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$.
                        \item If $(X_k, X_p)$ is a direct relation, $X_{p}$ must not be a collider, and $X_i \indep X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$.
                    \end{itemize}
                
                    \item The case where $p > k$. In this case, $(X_k, X_p)$ can only be a confounded pair. Because of assumption \ref{assum:t2a2}, $X_k$ and $X_p$ cannot be caused by another confounder or higher-order direct relation. Therefore, there must be $\{X_i \rightarrow X_k\}$ and $k = i+1$ for the path to be d-connected. We further discuss the following cases:
                    \begin{itemize}
                        \item If $k< p < j$, because of assumption \ref{assum:t2a2}, $X_p$ cannot be caused by another confounder or higher-order direct relation. If $X_p$ is a collider, $X_{p-1}$ must not be a collider on the path as $\{X_{p-1} \rightarrow X_p\}$. Thus, we have $X_i \indep X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$.
                        \item If $p = j$, then $X_i \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$ because of $(X_{i+1}, X_{j})_c$, which implies $(X_i, X_j)_d \in \mathbf{E}_1$.
                        \item If $p > j$ ($X_p \notin \mathbf{X}_{\text{Pre}(j) \setminus i}$), the only case where the path between $X_i$ and $X_j$ is not d-seperated by $X_p$ is the case where $X_p$ is the cause of a selection variable. However, the index $p$ has already been included in $R[i]$ according to the order of tests in the algorithm (Lines 7-9, 16). According to assumption \ref{assum:t1a1}, $X_p$ cannot be caused by more than two observed variables via higher-order direct relations. Therefore, the only case for $X_i$ to be conditionally dependent of $X_j$ given $\{\mathbf{X}_{\text{Pre}(j) \setminus i}, X_{j+1}, X_k\}$ for all $k \in \mathcal{R}[i]$ is the structure that $\{X_i \rightarrow S \leftarrow X_p\}$ and $p = j+1$. However, this contradicts with assumption \ref{assum:t2a2} since $\{X_{i+1}, X_p\}$ is a confounded pair.
                        
                        % At the same time, if $\{X_i \rightarrow S \leftarrow X_p\}$ and $p = j+1$, we also have $X_i \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$ because of $(X_i, X_{j+1})_s$. As a result, we have $(X_i, X_j)_d \in \mathbf{E}_1$.
                    \end{itemize}
                    
                \end{itemize}
                
            \item The case where $k > j$. If $k > j$ ($X_k \notin \mathbf{X}_{\text{Pre}(j) \setminus i}$), the only case where the path between $X_i$ and $X_j$ is not d-seperated by $X_k$ is the case where $X_k$ is the cause of a selection variable. However, since we have $\{X_i \cdots \rightarrow X_k\}$, it is not possible for $(X_i, X_k)$ to be a selection pair. For any other selection pairs, in order to have $X_i \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$, $(X_j, X_k)$ must be a selection pair. According to assumption \ref{assum:t1a1}, we have $k \neq j+1$. Therefore, the path is d-seperated by either $k$, where $k \in \mathcal{R}[i]$, or $j+1$. Consequently, there must be the conditional independence $X_i \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}, X_{j+1}, X_k\}$ and thus $(X_i, X_j)_d \notin \mathbf{E}_1$.
        \end{itemize}


        \item $\{X_i \cdots \leftrightarrow X_k \cdots X_j\}$, where $k>i$. Based on this, we discuss the following cases:
        \begin{itemize}
            \item The case where $i < k < j$. Since $\mathbf{X}_{\text{Pre}(j) \setminus i}$ is the condition set and $X_k \in \mathbf{X}_{\text{Pre}(j) \setminus i}$, $X_k$ must be a collider for the path to be d-connected. At the same time $(X_i, X_k)$ must be a selection pair. We further discuss the following cases:
                \begin{itemize}
                    \item The case where $k = i+1$. According to assumption \ref{assum:t1a1}, $(X_i, X_k)$ cannot be a selection pair if $k = i+1$, which is a contradiction.
                    \item The case where $k \neq i+1$. On the path, let us denote the $X_p$ as the observed variable closest to $X_k$ other than $X_i$. Thus, we must have $\{X_k \leftarrow \cdots X_p\}$ on the path. We further have the following cases:
                     \begin{itemize}
                        \item The case where $p < k$. If $p < k$, we have $p < i$ as $p \neq i$. Since $\{X_k \leftarrow \cdots X_p\}$, $(X_k, X_p)$ is either a confounded pair or direct relation. If $(X_k, X_p)$ is a confounded pair, because $X_p$ cannot be caused by another confounder (assumption \ref{assum:t2a2}), the only case for $X_p$ to also be a collider is $\{X_k \leftarrow C \rightarrow X_p \leftarrow X_{p-1}\}$. Thus, $X_{p-1}$ must not be a collider, and $X_i \indep X_j |\{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$; If $(X_k, X_p)$ is a direct relation, $X_{p}$ must not be a collider, and $X_i \indep X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$.
                        % \begin{itemize}
                        %     \item If $(X_k, X_p)$ is a confounded pair, because $X_p$ cannot be caused by another confounder (assumption \ref{assum:t2a2}), the only case for $X_p$ to also be a collider is $\{X_k \leftarrow C \rightarrow X_p \leftarrow X_{p-1}\}$. Thus, $X_{p-1}$ must not be a collider, and $X_i \indep X_j |\{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$.
                        %     \item If $(X_k, X_p)$ is a direct relation, $X_{p}$ must not be a collider, and $X_i \indep X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$, which implies $(X_i, X_j)_d \notin \mathbf{E}_1$.
                        % \end{itemize}               
                        \item The case where $p > k$. In this case, $(X_k, X_p)$ can only be a confounded pair. However, because $k \neq i+1$ and $\{X_i \cdots \leftrightarrow X_k \}$, $(X_i, X_k)$ is either a confounded pair or higher-order direct relation, both of which are impossible according to assumption \ref{assum:t2a2}. Thus, $(X_i, X_j)_d \notin \mathbf{E}_1$.
                    \end{itemize}               
                \end{itemize}
            \item The case where $k > j$. If $k > j$ ($X_k \notin \mathbf{X}_{\text{Pre}(j) \setminus i}$), the only case where the path between $X_i$ and $X_j$ is not d-seperated by $X_k$ is the case where $X_k$ is the cause of a selection variable. However, the index $k$ for any selection pair $\{X_{i}, X_k\}_s$, where $k>j$, has already been included in $R[i]$ according to the order of tests in the algorithm (Lines 7-9, 16). According to assumption \ref{assum:t1a1}, $X_k$ cannot be caused by more than two observed variables via higher-order direct relations. Therefore, the only case for $X_i$ to be conditionally dependent of $X_j$ given $\{\mathbf{X}_{\text{Pre}(j) \setminus i}, X_{j+1}, X_k\}$ for all $k \in \mathcal{R}[i]$ is the structure that $(X_i, X_{j+1})_{\{s,x\}}$. At the same time, we also have $X_i \notindependent X_j | \{\mathbf{X}_{\text{Pre}(j) \setminus i}\}$. As a result, we have $(X_i, X_j)_d \in \mathbf{E}_1$.
        \end{itemize}
    \end{itemize}

    \textbf{Stage II.} \ \ 
    Next, we prove that we can identify selection pairs, direct relations, and dependent pairs that are both selection pairs and direct relations in $\mathcal{E}_1$ after Lines 19-45 in the algorithm. At the same time, we can also identify and remove spurious dependent pairs $(X_i, X_j)$ that there exists $(X_i, X_{j+1})_{\{s,x\}}$ in the ground-truth graph. After this stage, there are still some spurious dependent pairs because of unidentified confounded pairs. Note that, according to the algorithm, for any $X_i$, the tests start from variables in $\mathcal{R}[i]$ with the largest index and continue in a descending order. In addition, $X_k$ for $k$ after lines (23,24) is a variable where $(X_i, X_k)$ is not a pair in $\mathcal{E}_1$. 
    
    We discuss the following cases for all types in $\mathcal{E}_1$.
        \begin{itemize}
            \item $(X_i, X_j)$ is a selection pair but not a direct relation. According to the algorithm, it will be identified as a selection pair but not a direct relation if and only if $\exists v \in \mathbf{T}_1$, $X_i \indep X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}$, where $X_v$ is a variable in any potential selection pair $(X_i, X_v)$ where $v > j$ (the definition of $\mathbf{T}_1$ is in Line 26 in the algorithm). Note that $j \in \mathcalk{R}[j-1]$ and $j+1 \notin \mathcalk{R}[i]$ according to assumption \ref{assum:t1a1}. 

            % In this case, according to assumption \ref{assum:t1a1}, for any $p$ where $k < p < j$, $(X_i, X_p)$ must not be a selection pair. Therefore, we have $X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j\}$ for $(X_i, X_j)_s$.
            
            % In addition, for any potential selection pair $(X_i, X_v)$ where $v > j$, it is included in $\mathbf{T}_1$ defined in Line 26 in the algorithm. At the same time, $X_v$ cannot be caused by 
            
            % Thus, for all $X_v \in \mathbf{T}_1$, we also have 
            
            Suppose that there exist a path other than $\{X_i \rightarrow S \leftarrow X_j \cdots X_k\}$ that makes $X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}, \forall v \in \mathbf{T}_1$. We discuss all potential cases for that path:
            \begin{itemize}
                \item $\{X_i \cdots \leftarrow X_p \cdots X_k\}$, where $p<i$ and $X_p$ denotes the observed variable that is the closest to $X_i$ on the path. Since $X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$, this path is d-connected if and only if $X_p$ is a collider on the path. However, $X_p$ cannot be a collider because of $\{X_i \leftarrow X_p\}$. Thus, this case is impossible.
                \item $\{X_i \cdots \rightarrow X_p \cdots X_k\}$, where $p<i$ and $X_p$ denotes the observed variable that is the closest to $X_i$ on the path. Because of assumption \ref{assum:t2a1}, $\{X_i \rightarrow X_p\}$ is impossible. Thus, there must be a confounded pair $\{X_i, X_p\}_c$. Because of assumption \ref{assum:t2a2}, $X_p$ cannot be caused by another confounder or observed variable via higher-order direct relation. Therefore, $X_p$ is not a collider and this case is impossible
                \item $\{X_i \cdots \leftrightarrow X_p \cdots X_k\}$, where $p<i$ and $X_p$ denotes the observed variable that is the closest to $X_i$ on the path. Because of assumption \ref{assum:t2a1}, $\{X_i \rightarrow X_p\}$ is impossible. Thus, there must be a confounded pair $\{X_p, X_i\}_c$. Because of assumption \ref{assum:t2a2}, $(X_p, X_i)$ cannot be a selection pair or direct relation, and $X_p$ cannot be caused by another confounder or observed variable via higher-order direct relation. We further discuss the following cases:
                \begin{itemize}
                    \item $X_p$ is a collider. For $X_p$ to be a collider, the only case is $\{X_{p-1} \rightarrow X_p \leftarrow C \rightarrow X_i\}$, where $C$ as the corresponding latent confounder in $\mathbf{C}$. In that case, $X_{p-1} \in \mathbf{X}_{\text{Pre}(k) \setminus i}$ cannot be a collider on the path. Thus, this case is impossible.
                    \item $X_p$ is not a collider. Then we have $X_i \indep X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}, \forall v \in \mathbf{T}_1$ ($X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$) and thus this case is impossible.
                \end{itemize}
           
                \item $\{X_i \cdots \leftarrow X_p \cdots X_k\}$, where $i < p < k$ and $X_p$ denotes the observed variable that is the closest to $X_i$ on the path. Because of assumption \ref{assum:t2a1}, $\{X_i \leftarrow X_p\}$ is impossible. Thus, there must be a selection pair $(X_i, X_p)_s$, and $X_p$ must not be a collider. Since $\{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}$ is the condition set and $X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$, we have $X_i \indep X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}, \forall v \in \mathbf{T}_1$ ($X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$) and thus this case is impossible.

                \item $\{X_i \cdots \rightarrow X_p \cdots X_k\}$, where $i < p < k$. Since $\mathbf{X}_{\text{Pre}(k) \setminus i}$ is in the condition set and $X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$, $X_p$ must be a collider for the path to be d-connected. On the path, let us denote the $X_q$ as the observed variable closest to $X_p$ other than $X_i$. Thus, we must have $\{X_p \leftarrow \cdots X_q\}$ on the path. We further have the following cases:
                    \begin{itemize}
                    \item The case where $q < p$. If $q < p$, we have $q < i$ as $q \neq i$. Since $\{X_p \leftarrow \cdots X_q\}$, $(X_p, X_q)$ is either a confounded pair or direct relation. We further discuss the following cases:
                    \begin{itemize}
                        \item If $(X_p, X_q)$ is a confounded pair, because $X_q$ cannot be caused by another confounder (assumption \ref{assum:t2a2}), the only case for $X_q$ to also be a collider is $\{X_p \leftarrow C \rightarrow X_q \leftarrow X_{q-1}$. Thus, $X_{q-1}$ must not be a collider, and $X_i \indep X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}, \forall v \in \mathbf{T}_1$ ($X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$) and thus this case is impossible.
                        \item If $(X_p, X_q)$ is a direct relation, $X_{q}$ must not be a collider, and $X_i \indep X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}, \forall v \in \mathbf{T}_1$ ($X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$) and thus this case is impossible.
                    \end{itemize}
                
                    \item The case where $q > p$. In this case, $(X_p, X_q)$ can only be a confounded pair. Because of assumption \ref{assum:t2a2}, $X_p$ and $X_q$ cannot be caused by another confounder or higher-order direct relation. Therefore, there must be $\{X_i \rightarrow X_p\}$ and $p = i+1$ for the path to be d-connected. We further discuss the following cases:
                    \begin{itemize}
                        \item If $p < q < k$, because of assumption \ref{assum:t2a2}, $X_q$ cannot be caused by another confounder or higher-order direct relation. If $X_q$ is a collider, $X_{q-1}$ must not be a collider on the path as $\{X_{q-1} \rightarrow X_q\}$, and $X_i \indep X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}, \forall v \in \mathbf{T}_1$ ($X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$) and thus this case is impossible.
                        \item If $q = k$, then we have $(X_{i+1}, X_{k})_c$, which is a contradiction to the definition of $k$ ($k \in \mathcal{R}[i]$ according to the algorithm)
                        \item If $k < q < j$, because of assumption \ref{assum:t2a2}, $(X_{p-1}, X_{q+1})_{d\neq c}$ should not exist. However, since $p-1 = i$, this contradicts the definition of $k$ ($k \in \mathcal{R}[i]$ according to the algorithm) or the existing selection pair $(X_i, X_j)_s$.
                        \item If $q = j$, this contradicts assumption \ref{assum:t2a2} that there exists no $(X_i, X_j)_s$ ($i = p-1$).
                        \item If $q > j$, if not conditioning on $X_q$, the only case where the path between $X_i$ and $X_k$ is not d-seperated by $X_q$ is the case where $X_q$ is the cause of a selection variable. However, the index $q$ has already been included in $R[i]$ according to the order of tests in the algorithm (Lines 20-21). According to assumption \ref{assum:t1a1}, $X_q$ cannot be caused by more than two observed variables via higher-order direct relations. As a result, we have $X_i \indep X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}, \forall v \in \mathbf{T}_1$ ($X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$) and thus this case is impossible.
                    \end{itemize}   
                \end{itemize}


                \item $\{X_i \cdots \leftrightarrow X_p \cdots X_k\}$, where $i < p < k$. Since $\mathbf{X}_{\text{Pre}(k) \setminus i}$ is in the condition set and $X_p \in \mathbf{X}_{\text{Pre}(k) \setminus i}$, $X_p$ must be a collider for the path to be d-connected. At the same time $(X_i, X_p)$ must be a selection pair. We further discuss the following cases:
                \begin{itemize}
                    \item The case where $p = i+1$. According to assumption \ref{assum:t1a1}, $(X_i, X_p)$ cannot be a selection pair if $p = i+1$, which is a contradiction.
                    \item The case where $p \neq i+1$. On the path, let us denote the $X_q$ as the observed variable closest to $X_p$ other than $X_i$. Thus, we must have $\{X_p \leftarrow \cdots X_q\}$ on the path. We further have the following cases:
                     \begin{itemize}
                        \item The case where $q < p$. If $q < p$, we have $q < i$ as $q \neq i$. Since $\{X_p \leftarrow \cdots X_q\}$, $(X_q, X_p)$ is either a confounded pair or direct relation. If $(X_q, X_p)$ is a confounded pair, because $X_q$ cannot be caused by another confounder (assumption \ref{assum:t2a2}), the only case for $X_q$ to also be a collider is $\{X_p \leftarrow C \rightarrow X_q \leftarrow X_{q-1}\}$. Thus, $X_{q-1}$ must not be a collider, and the path is not d-connected; If $(X_q, X_p)$ is a direct relation, $X_{q}$ must not be a collider, and the path is, again, not d-connected. Thus, this case is impossible.
                        \item The case where $q > p$. In this case, $(X_p, X_q)$ can only be a confounded pair. However, because $p \neq i+1$ and $\{X_i \cdots \leftrightarrow X_p \}$, $(X_i, X_p)$ is either a confounded pair or higher-order direct relation, both of which are impossible according to assumption \ref{assum:t2a2}. Thus, this case is impossible.
                    \end{itemize}               
                \end{itemize}
                
                \item $\{X_i \cdots \leftarrow X_p\}$, where $k=p$. This is impossible because of the algorithm, specifically, how $k$ is selected (lines 20-25).

                \item $\{X_i \cdots \rightarrow X_p\}$, where $k=p$. This is also impossible because of the algorithm.

                \item $\{X_i \cdots \leftrightarrow X_p\}$, where $k=p$. Similarly, this is impossible according to the algorithm.

                \item $\{X_i \cdots \leftarrow X_p \cdots X_k\}$, $k < p < j$. Because of assumption \ref{assum:t2a1}, $\{X_i \leftarrow X_p\}$ is impossible. Thus, there must be a selection pair $(X_i, X_p)_s$. 
                % According to assumptions \ref{assum:t2a1} and \ref{assum:t2a2}, if $(X_i, X_p)$ is a selection pair, then it is impossible for $(X_i, X_{p+1})$ to be a dependent pair and $(X_{i+1}, X_{p+1})$ to be a confounded pair.
                Together with the search procedure (lines 20-25), it is thus impossible for the selected $k$ to be smaller than $p$, which is a contradiction.

                \item $\{X_i \cdots \rightarrow X_p \cdots X_k\}$, $k < p < j$. Because of $\{X_i \cdots \rightarrow X_p\}$, $(X_i, X_p)$ is either a higher-order direct relation or a confounded pair. Since $X_p$ is not in the condition set, $(X_i, X_p)$ must also be a selection pair for the path to be d-connected. However, according to assumption \ref{assum:t1a1}, there exits no $(X_i, X_{p+1})_d$. This contradicts the search procedure to select $k$ (lines 20-25), and thus this case is impossible.

                \item $\{X_i \cdots \leftrightarrow X_p \cdots X_k\}$, $k < p < j$. Because of assumption \ref{assum:t2a1}, $\{X_i \leftarrow X_p\}$ is impossible. Thus, there must be a selection pair $(X_i, X_p)_s$. Thus, there must be a selection pair $(X_i, X_p)_s$. Similarly, it is thus impossible for the selected $k$ to be smaller than $p$, which is a contradiction.
          
            \end{itemize}
            Therefore, there does not exist any path other than $\{X_i \rightarrow S \leftarrow X_j \cdots X_k\}$ that makes $X_i \notindependent X_k | \{\mathbf{X}_{\text{Pre}(k) \setminus i}, X_j, X_v\}, \forall v \in \mathbf{T}_1$. 
           
            \item $(X_i, X_j)$ is a direct relation but not a selection pair.
            \item $(X_i, X_j)$ is both a selection pair and a direct relation.
            \item $(X_i, X_j)$ is a confounded pair.
            \item $(X_i, X_j)$ is a spurious dependent pair that there exist a confounded pair $(X_{i+1}, X_j)_c$ in the ground-truth causal graph.
            \item $(X_i, X_j)$ is a spurious dependent pair that there exist $(X_i, X_{j+1})$ that is both a selection pair and a direct relation in the ground-truth causal graph. 
        \end{itemize}
        
    
    % At the same time, it is also necessary to show that there are no other types of variable pairs included in the identified sets in the identified set $\mathbf{E}_1$. Suppose there exists a variable pair $(X_k, X_v) \in \mathbf{E}_1$ i.e. not any of the types listed above. Without the loss of generality, we assume $k < v$.
    % \begin{itemize}
    %     \item If $(X_k, X_v)$ is not a dependent pair (selection pair, direct relation, or confounded pair), then $X_k$ is not dependent with 
    %     the only possibility that $X_i \notindependent X_j | \mathbf{X}_{\text{Pre}(j) \setminus i}$  
    % \end{itemize}
\end{proof}
